Spectral Statistics of the Sample Covariance Matrix for High Dimensional Linear Gaussians

Performance of ordinary least squares(OLS) method for the \emph{estimation of high dimensional stable state transition matrix} $A$(i.e., spectral radius $\rho(A)<1$) from a single noisy observed trajectory of the linear time invariant(LTI)\footnote{Linear Gaussian (LG) in Markov chain literature} system $X_{-}:(x_0,x_1, \ldots,x_{N-1})$ satisfying \begin{equation} x_{t+1}=Ax_{t}+w_{t}, \hspace{10pt} \text{ where } w_{t} \thicksim N(0,I_{n}), \end{equation} heavily rely on negative moments of the sample covariance matrix: $(X_{-}X_{-}^{*})=\sum_{i=0}^{N-1}x_{i}x_{i}^{*}$ and singular values of $EX_{-}^{*}$, where $E$ is a rectangular Gaussian ensemble $E=[w_0, \ldots, w_{N-1}]$. Negative moments requires sharp estimates on all the eigenvalues $\lambda_{1}\big(X_{-}X_{-}^{*}\big) \geq \ldots \geq \lambda_{n}\big(X_{-}X_{-}^{*}\big) \geq 0$. Leveraging upon recent results on spectral theorem for non-Hermitian operators in \cite{naeem2023spectral}, along with concentration of measure phenomenon and perturbation theory(Gershgorins' and Cauchys' interlacing theorem) we show that only when $A=A^{*}$, typical order of $\lambda_{j}\big(X_{-}X_{-}^{*}\big) \in \big[N-n\sqrt{N}, N+n\sqrt{N}\big]$ for all $j \in [n]$. However, in \emph{high dimensions} when $A$ has only one distinct eigenvalue $\lambda$ with geometric multiplicity of one, then as soon as eigenvalue leaves \emph{complex half unit disc}, largest eigenvalue suffers from curse of dimensionality: $\lambda_{1}\big(X_{-}X_{-}^{*}\big)=\Omega\big( \lfloor\frac{N}{n}\rfloor e^{\alpha_{\lambda}n} \big)$, while smallest eigenvalue $\lambda_{n}\big(X_{-}X_{-}^{*}\big) \in (0, N+\sqrt{N}]$. Consequently, OLS estimator incurs a \emph{phase transition} and becomes \emph{transient: increasing iteration only worsens estimation error}, all of this happening when the dynamics are generated from stable systems.

==> elementwise.tex <==
\section{Elementwise estimation error}
\label{sec:exactOLS}
Although, bounds on estimation error discussed in preceding section provide a good intuition, but existing analysis based on martingales e.t.c does not reveal explicit dependencies on number of iterations and state space dimensions. Surprisingly, it had been left unnoticed that pseudo-inverse is constrained with respect to the data matrix which we discussed is itself a function of Gaussian ensemble $E$ and element-wise estimation error is an inner product between Gaussian ensemble and pseudo-inverse.

% \textcolor{red}{check if move from $x_{i}$ to $x_{i-1}$}
\begin{theorem}
\label{thm:invcovneg2ndmoment}[Construction of Inverse Sample Covariance Matrix]
Let $[e_{j}]_{j=1}^{n}$ be canonical basis of $\mathbb{C}^{n}$ and $X_{-}$ be the data matrix of stable linear dynamical system with isotropic Gaussian noise as in \eqref{eq:LGS}, Given, the rows of data matrix $[y_{j}]_{j=1}^{n}$, inverse sample covariance matrix $\big(X_{-}X_{-}^{*}\big)^{-1}=[v_{j,k}]_{j,k=1}^{n}$ satisfies following constraints:
\begin{enumerate}
    \item For fixed $j$ in $[1, \ldots, n]$, $\sum_{k \neq j} v_{j,k} \big\langle y_{k},y_{j} \big\rangle=1- v_{j,j}\|y_{j}\|^{2}$, precisely said:
    \begin{align}
        & \label{eq:lin1} \sum_{k \neq j} v_{j,k} \sum_{i=1}^{N-1} \sum_{t=1}^{i}\big \langle A^{i-t} w_{t-1},e_{k} \big \rangle \overline{\sum_{t=1}^{i}\big \langle A^{i-t}w_{t-1},e_{j} \big \rangle} = 1-v_{j,j}\sum_{i=1}^{N-1} \bigg| \sum_{t=1}^{i}\big \langle A^{i-t} w_{t-1},e_{j} \big \rangle \bigg|^{2}
    \end{align}
    \item and for all $l \neq j$, $\sum_{k=1}^{n} v_{j,k} \big\langle y_{k},y_{l} \big\rangle=0$, precisely said:
    \begin{align}
    \nonumber \sum_{k=1}^{n} v_{j,k}\sum_{i=1}^{N-1} &\sum_{t=1}^{i}\big \langle A^{i-t}w_{t-1},e_{k} \big \rangle \overline{\sum_{t=1}^{i}\big \langle A^{i-t}w_{t-1},e_{l} \big \rangle}\\ & \label{eq:lin2}=0 
    \end{align}
    \item diagonal entries of inverse sample covariance matrix are inverse  distance squared  between row and conjugate hyperplane, to be precise: 
    \begin{align}
    \label{eq:invsmpdiag} \bigg \langle (\sum_{t=0}^{N-1}x_{t}x_{t}^{*})^{-1} e_{j}  ,e_{j}\bigg\rangle= \frac{1}{d^{2}(y_j,n_j)}=v_{j,j},  
    \end{align}
\end{enumerate} 
\end{theorem}
\begin{proof}
We follow the direction given in \cite{tao2010random}, let $v_{j}:=\big(X_{-}X_{-}^{*}\big)^{-1}e_{j}$, in columns format we have $X_{-}^{*}=[y_1,\ldots,y_{n}]$, $X_{-}^{*} e_{j}=y_{j}$, $n_{j}=$span$[y_{i}]_{i \neq j}$.
\begin{align}
 & \label{eq:deltajk} \bigg\langle X_{-}^{*} \big(X_{-}X_{-}^{*}\big)^{-1}e_{j},X_{-}^{*}e_{k}\bigg \rangle =\delta_{j}(k)
\end{align}
Notice that inner product of $X_{-}^{*} \big(X_{-}X_{-}^{*}\big)^{-1}e_{j}$ with $X_{-}^{*}e_{k}=:y_{k}$ for $k \neq j$ is zero; so for each $j \in [n]$ , $X_{-}^{*} \big(X_{-}X_{-}^{*}\big)^{-1}e_{j}$ is orthogonal to $n_{j}$. Since,
\begin{equation}
    X_{-}^{*}v_{j}=v_{j,1}y_1+\ldots+v_{j,n}y_{n},
\end{equation}
\eqref{eq:lin1} and \eqref{eq:lin2} readily follows. As   $X_{-}^{*} \big(X_{-}X_{-}^{*}\big)^{-1}e_{j}$ is orthogonal to $n_{j}$, according to  Corollary \ref{cor:vimpescpnegmomstuck} 
\begin{equation}
    \big\langle X_{-}^{*} \big(X_{-}X_{-}^{*}\big)^{-1}e_{j},X_{-}^{*}e_{j}\big\rangle = \big\langle X_{-}^{*} 
    \big(X_{-}X_{-}^{*}\big)^{-1}e_{j},P_{n_j^{\perp}}(X_{-}^{*}e_{j})\big\rangle
\end{equation}
Furthermore, using \eqref{eq:deltajk} and properties of orthogonal projection:
\begin{align}
     \nonumber 1 &=\big\langle X_{-}^{*} \big(X_{-}X_{-}^{*}\big)^{-1}e_{j},X_{-}^{*}e_{j}\big\rangle = \big\langle X_{-}^{*}\big(X_{-}X_{-}^{*}\big)^{-1}e_{j},P_{n_j^{\perp}}(X_{-}^{*}e_{j})\big\rangle    \big\langle P_{n_j^{\perp}}\big[X_{-}^{*} \big(X_{-}X_{-}^{*}\big)^{-1}e_{j}\big],X_{-}^{*}e_{j}\big\rangle\\ & = \sum_{i\neq j}^{n} v_{j,i}\big\langle \underbrace{P_{n_j^{\perp}}y_{i}}_{=0}, y_{j}\big \rangle  +\nonumber v_{j,j}\langle P_{n_j^{\perp}} y_{j} , y_{j}\rangle  =v_{j,j}\langle P_{n_j^{\perp}} y_{j}, P_{n_j^{\perp}} y_{j}\rangle =v_{j,j} \|P_{n_j^{\perp}} y_{j}\|^{2} =v_{j,j}d^{2}(y_{j},n_{j}). \hspace{10pt} 
\end{align}
Therefore, $v_{j,j}=\frac{1}{d^{2}(y_{j},n_{j})}$
\end{proof}
\begin{remark}
 Notice that total number of unknowns $v_{j,k}$ are $\frac{n(n+1)}{2}$ which equals distinct interaction potentials of observations$\langle y_{j}, y_{k}\rangle$. A remarkable advantage of enlisting these constraints is when we do not have independence between the rows as in Hermitian case, we still have:
\begin{align}
     & \nonumber d_{j}^{-2}=\frac{1-\sum_{k \neq j} v_{j,k} \langle y_{k} , y_{j} \rangle}{\|y_{j}\|^{2}},\textit{where} \hspace{3pt}  \sum_{k \neq j} v_{j,k} \langle   y_{k} , y_{j} \rangle \leq 0 \hspace{3pt} \textit{and} \\ &\sum_{j=1}^{n} d_{j}^{-2}= \frac{\sum_{j=1}^{n} \prod_{l \neq j} \|y_{l}\|^{2}\big(1-\sum_{k \neq j} v_{j,k} \langle y_{k} , y_{j} \rangle \big)    }{\prod_{j=1}^{n} \|y_{j}\|^{2}}  
\end{align} 
\end{remark}
\begin{itemize}
    \item Dimension, $n=2$ precision matrix: 
    \begin{align}
    & \label{eq:dim2precisionmatrxi} v_{1,1}\|y_1\|^{2}+v_{1,2}\langle y_2,y_1\rangle=1 \\ & \nonumber v_{2,2}\|y_2\|^{2}+v_{2,1} \langle y_1,y_2\rangle=1 \\ & \nonumber v_{1,1} \langle y_1 , y_2\rangle +v_{1,2} \|y_2\|^{2}=0 \\ & \nonumber v_{2,1}\|y_1\|^{2}+v_{2,2} \langle y_2,y_1 \rangle =0.
    \end{align}
    First two equations imply that
    \begin{equation}
        \frac{v_{1,1}}{v_{2,2}}=\frac{\|y_2\|^{2}}{\|y_1\|^2}.
    \end{equation}
    and combined with the third we have:
    \begin{equation}
        v_{1,2}\|y_2\|^{2}=-v_{1,1} \langle y_1,y_2\rangle \hspace{3pt} \implies 
    \end{equation}
\end{itemize}

\begin{enumerate}
    \item For fixed $j$ in $[1, \ldots, n]$ and $N$, 
    \begin{align}
        \nonumber  \frac{\|y_{j}\|^{2}}{d^{2}(y_j,n_j)}=1-\sum_{k \neq j}\big\langle  v_{j,k} y_{k} , y_{j} \big\rangle&= 1-v_{j,1}\langle y_1 ,y_j \rangle +\ldots+v_{j,j-1}\langle y_{j-1} ,y_j \rangle \\ & \nonumber+v_{j,j+1}\langle y_{j+1} ,y_j \rangle+ \ldots+ v_{j,n}\langle y_{n} ,y_j \rangle 
    \end{align}
     Pythagorous theorem implies $\frac{\|y_{j}\|^{2}}{d^{2}(y_j,n_{j})} \geq 1$, so regardless of the length of simulated trajectory $ \sum_{k \neq j} \big\langle  v_{j,k} y_{k} , y_{j} \big\rangle \leq 0$, precise expression $0\geq$ 
    \begin{align}
        & \label{eq:lin1} \sum_{k \neq j} v_{j,k}\sum_{i=1}^{N}\sum_{t',t=1}^{i} \sum_{m'=0}^{(i-t') \land (n-j) } \sum_{m=0}^{(i-t) \land (n-k) } \binom{i-t'}{m'}\binom{i-t}{m} \lambda^{2i-(t'+t)-(m'+m)} \langle w_{t'-1} ,e_{m'+j}  \rangle \langle w_{t-1} ,e_{m+k}  \rangle   
    \end{align}
     
    \item and for all $l \neq j$, $\sum_{k=1}^{n} v_{j,k} \big\langle y_{k},y_{l} \big\rangle=0$, precisely said $0=$
    \begin{align}
    & \label{eq:lin2}  \sum_{k=1}^{n} v_{j,k} \sum_{i=1}^{N}\sum_{t',t=1}^{i} \sum_{m'=0}^{(i-t') \land (n-l) }  \sum_{m=0}^{(i-t) \land (n-k) } \binom{i-t'}{m'}\binom{i-t}{m} \lambda^{2i-(t'+t)-(m'+m)} \langle w_{t'-1} ,e_{m'+l} \rangle \langle w_{t-1} ,e_{m+k}  \rangle  .  
    \end{align}
    \item diagonal entries of inverse sample covariance matrix are inverse  distance squared  between row and conjugate hyperplane, to be precise: 
    \begin{align}
    \label{eq:invsmpdiag} \bigg \langle (\sum_{t=0}^{N-1}x_{t}x_{t}^{*})^{-1} e_{j}  ,e_{j}\bigg\rangle= \frac{1}{d^{2}(y_j,v_j)}=v_{j,j},  
    \end{align}
\end{enumerate} 
\begin{align}
    
& \nonumber \big\|A-\hat{A} \big\|_{F} \leq \sigma_{1}(EX_{-}^{*}) \sqrt{\sum_{j=1}^{n} \frac{1}{\sigma_{j}^{4}(X_{-})}}=\sqrt{\sum_{j=1}^{n} \frac{n\sigma_{1}^{2}(X_{-})}{\sigma_{j}^{4}(X_{-})}}=\sqrt{\sum_{j=1}^{n} \frac{n\sigma_{1}^{2}(X_{-})}{\sigma_{j}^{4}(X_{-})}}=\sqrt{\frac{n}{\sigma_{1}^{2}}+\sum_{j=2}^{n} \frac{n\sigma_{1}^{2}(X_{-})}{\sigma_{j}^{4}(X_{-})}} \\ & \nonumber \sqrt{\frac{n}{\sigma_{1}^{2}}+ \frac{n \sigma_{1}^{2}}{\sigma_{2}^{4}}+\sum_{j=3}^{n} \frac{n\sigma_{1}^{2}(X_{-})}{\sigma_{j}^{4}(X_{-})}}  \\ & \nonumber
    \sum_{j=1}^{n} \frac{1}{\sigma_{j}^{2}(X_{-})} \leq \sqrt{\sum_{j=1}^{n} \frac{n}{\sigma_{j}^{4}(X_{-})}}, \hspace{5pt} \big\|A-\hat{A} \big\|_{F} \leq \sqrt{\sum_{j=1}^{n} \frac{n}{\sigma_{j}^{2}(X_{-})}}      
    \end{align}
